Comparison between an exact and a heuristic neural mass model with second order synapses

Neural mass models (NMMs) are designed to reproduce the collective dynamics of neuronal populations. A common framework for NMMs assumes heuristically that the output firing rate of a neural population can be described by a static nonlinear transfer function (NMM1). However, a recent exact mean-field theory for quadratic integrate-and-fire (QIF) neurons challenges this view by showing that the mean firing rate is not a static function of the neuronal state but follows two coupled nonlinear differential equations (NMM2). Here we analyze and compare these two descriptions in the presence of second-order synaptic dynamics. First, we derive the mathematical equivalence between the two models in the infinitely slow synapse limit, i.e., we show that NMM1 is an approximation of NMM2 in this regime. Next, we evaluate the applicability of this limit in the context of realistic physiological parameter values by analyzing the dynamics of models with inhibitory or excitatory synapses. We show that NMM1 fails to reproduce important dynamical features of the exact model, such as the self-sustained oscillations of an inhibitory interneuron QIF network. Furthermore, in the exact model but not in the limit one, stimulation of a pyramidal cell population induces resonant oscillatory activity whose peak frequency and amplitude increase with the self-coupling gain and the external excitatory input. This may play a role in the enhanced response of densely connected networks to weak uniform inputs, such as the electric fields produced by non-invasive brain stimulation.

==> old_references_and_tables/old_abstract.tex <==
Neural mass models (NMMs) are low-dimensional representations of the dynamics of populations of neurons.
They are usually constructed from heuristic assumptions by combining second-order linear dynamics for the average post-synaptic potential with a nonlinear transfer function providing the mean firing rate response of a neural population as a function of the total membrane potential alteration.

However, a recent mean-field theory for quadratic integrate-and-fire (QIF) neurons challenges this framework by showing that, rather than a static function,  the low-dimensional firing rate dynamics of a neural population is described by two coupled nonlinear differential equations. 
In this paper we focus on an extension of this theory by adding second order synaptic dynamics and interaction with an external electric field to a single population of either excitatory or inhibitory neurons.
The resulting model, which we refer to as NMM2, contains two time scales, one for the membrane dynamics and one for the synaptic activity.
We show that, in the limit of slow synapses and external inputs, the NMM2 equations reduce to a simpler model with a static transfer function.
However, review of physiological literature illustrates that, in realistic situations, this limit may often be out of reach, and thus the full NMM2 equations should be used.
For example, bifurcation analysis unveils that the NMM2 population displays interneuron gamma oscillations, a state that is not described by the reduced model.
Additionally, we show that the NMM2 population exhibits oscillatory transient dynamics which, under the
effect of electric stimulation, produces Arnold tongues with peak frequency and amplitude increased by the self-coupling gain and external
excitatory input.
This may play a role in  the enhanced response of densely connected networks to weak, uniform inputs such as the  electric fields produced by non-invasive brain stimulation.  
Finally, the  new, dynamic transfer function  also endows the NMM2 with a  form of ``inertia'', an intrinsic  delayed response to external inputs that depends on, e.g.,  self-coupling strength and state of the system.

==> old_references_and_tables/tables.tex <==

%%%%%%%%%%%%%%%%
 \subsubsection{Relation of parameters to physiological data}
Table~\ref{table:nmm2parameters} provides an overview of the parameters in the QIF and NMM2 model in Equations~\ref{eq:qif} and~\ref{eq:nmm2}. Table~\ref{tab:tau} provides a more detailed analysis of the membrane and synaptic time constants for different populations. 


% %%%%%%%%%%%%%
% % PLACEHOLDER FOR TABLE

\begin{table*}[h!]
\begin{center}
\begin{tabular}{ | c |c | c | } 
  \hline
 {\bf  Symbol} & {\bf Units}  & {\bf Typical values} \\ 
  \hline
  $U_t-U_r$ & (potential) mV & 50--100  \\
  \hline
  $g_L$ & (conductance) S  & yyy--xxx  \\ 
    \hline
      $g_L(U_t-U_r)$ & (current) nA  & yyy--xxx  \\ 
    \hline
  $c$ & (capacitance) nF & 0.2--1.0  \\ 
      \hline
        $c(U_t-U_r)$ & (charge) pC & 10--100  \\ 
      \hline
  $\gamma$ & (charge) pC & 0.2--1.0  \\ 
  \hline
    $\kappa$ & (number of synapses) none & 0--10,000  \\ 
  \hline
 \hline
  $\varphi$, $s$ & (rate) Hz & 0--100 Hz \\ 
  \hline
  $J$ & (charge) none & 5--50  \cite{Jang:2010aa} \\ 
 \hline
  $\tau_m$ & (time) ms & 2--50    \\ 
 \hline
  $\tau_s$ & (time) ms & 2--50    \\ 
 \hline
  $\eta$ & (current) none & -5--5  \\ 
  \hline
    $\Delta$ & (current) none & (0,500] pA  \\ 
  \hline
\end{tabular} 
\end{center}
\caption{NMM2 variables, parameters with typical values and units in Equations~\ref{eq:qif} and~\ref{eq:nmm2}.}
\label{table:nmm2parameters}
\end{table*}

\begin{table}[h]
    \caption{Membrane time constants for different cell types \cite{neske2015,Zaitsev2012, Povysheva2007, Halabisky2006, Pronneke2015, Avermann2012, Manko2012, Olah2007, seay2020}}
    \centering
    \begin{tabular}{c|c|c|c|c |c | }
                     & PYR & PV & SST & VIP & NGFC \\\hline
%        $\tau_m$ (ms) & 11 & 4 & 11 & 11 & 9\\ 
%        $\tau_m$ (ms) & 19 & 9 & 19 & 19 & 13\\
        $\tau_m$ (ms) & 15 & 7.5 & 19 & 19 & 11\\
%        $\tau_m$ (ms) & 11 & \multicolumn{3}{c|}{13 $\pm$ 6} & 9\\\hline
        \end{tabular}
    \label{tab:taum}
\end{table}

\begin{table}[h]
    \caption{PSC time constants for different connections \cite{wonzy2011, karnani2016, bacci2003, Deleuze2019, bacci2003}}

    \centering
    \begin{tabular}{c|c}
    Neurotransmitter & $\tau_s$ \\\hline
     $\tau_{glu, PYR}$ (ms)& 10\\
    $\tau_{GABA,PV}$ (ms)& 2 \\
    $\tau_{GABA,SST}$ (ms)& 20\\
    $\tau_{GABA,VIP}$ (ms)& 25 \\
    $\tau_{GABA,NGFC}$ (ms)& 50 
    \end{tabular}
    \label{tab:taus}
\end{table}

\begin{table}[h]
    \caption{Coupling strength within and between populations (adapted from \cite{Jiang:2015aa})}
    \centering
    \begin{tabular}{c|c|c|c|c |c }
     From/to& PYR & PV   & SST & VIP & NGFC \\\hline
        PYR & low & high & low & low  & x\\
        PV  & medium & high & low &  low & low \\
        SST & medium & medium & x  & medium & medium \\
        VIP & x & x & medium & x & x\\
      NGFC & x & x & medium & x & x \\
        \end{tabular}

    \label{tab:coupling}
\end{table}

\begin{table}[h]
    \caption{Estimated percentages of the most significant synaptic connections in a cortical column (adapted from \cite{Jiang:2015aa, denoyer_modelling_2020, therewillbemorereferences})}
    \centering
    \begin{tabular}{c|c|c|c|c|c }
         Target & \multirow{2}{*}{PYR} & \multirow{2}{*}{PV} &  \multirow{2}{*}{SST} &  \multirow{2}{*}{VIP} &  \multirow{2}{*}{NGFC}  \\
         Source &  \\\hline
         PYR    & 66  & 70 & 71  & 53.75 & - \\
         PV     & 9.25 & 11.25 & - & - & - \\
         SST    & 6.5& 8.75 & - & 10.25& 33.5\\
         VIP    & - & - & 18 & - & - \\
         NGFC    & 4.75 & 1 & 4 & 2.75 & 34 \\\hline
         Thalomo-cortical & 1.35& 9&  7 & 33.25 & 32.5 \\\hline
         TOTAL & 100 & 100 & 100 & 100 & 100
         
    \end{tabular}
    \label{tab:connectivitypercentages}
\end{table}

%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsection{Effects of weak external field}
 
In \cite{Galan:2021aa} it is shown that in the linear regime (far from threshold) or when the electric vector field $E$ is weak, the effect of an electric field on  the membrane potential of a neuron compartment, or its average over a set of compartments, can be written in the form $V_E = \lambda \cdot E$, where $\lambda$ is a vector. This provides the rationale, inspired by experimental work, for the so-called ``lambda-E'' model used in transcranial electrical stimulation models \citep{ruffini_transcranial_2013,Ruffini:2014aa} and used in NMMs \citep{merlet_oscillatory_2013,molaee-ardekani_effects_2013}. This effect can also be described in terms of  the net axial current induced by the external field on the compartment or compartments describing the region of interest of the neuron, which provides the means for including the effect in the QIF model. That is, the effect of the electric field is associated to an input current into the QIF model which can be described in the passive regime with a dipole term $I_E = P\cdot E$. The region of interest in a realistic compartment neuron model can be taken to be the soma to compute the average net axial current for the QIF model \citep{Galan:2021aa}. Table~\ref{tab:electric} provides values for such perturbations from compartment models \citep{aberra_biophysically_2018,Galan:2021aa}.


\begin{table}[h]
    \caption{Effects of electric field of 1 V/m in soma \citep{aberra_biophysically_2018,Galan:2021aa} in terms of membrane potential alteration and equivalent input current.}
    \centering
    \begin{tabular}{c|c|c|c|c |c }
                      & PYR & PV & SST & VIP & NGFC \\\hline
        $V_E$ ($\mu$V)& 200 & 20 & 11 & 11 & 17\\
        $I_E$ (nA)& 10 & & & & - 
        \end{tabular}
    \label{tab:electric}
\end{table}
